Removing Local Extrema from Imprecise Terrains

In this paper we consider imprecise terrains, that is, triangulated terrains with a vertical error interval in the vertices. In particular, we study the problem of removing as many local extrema (minima and maxima) as possible from the terrain. We show that removing only minima or only maxima can be done optimally in O(n log n) time, for a terrain with n vertices. Interestingly, however, removing both the minima and maxima simultaneously is NP-hard, and is even hard to approximate within a factor of O(log log n) unless P=NP. Moreover, we show that even a simplified version of the problem where vertices can have only two different heights is already NP-hard, a result we obtain by proving hardness of a special case of 2-Disjoint Connected Subgraphs, a problem that has lately received considerable attention from the graph-algorithms community.

==> figures/bottom.pst.tex <==
% Generated with LaTeXDraw 2.0.2
% Fri Feb 12 09:22:29 CET 2010
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\begin{center}
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-0.96115)(9.2878,0.9721)
\definecolor{color835b}{rgb}{0.7568627450980392,0.8274509803921568,0.9411764705882353}
\definecolor{color3588b}{rgb}{0.7058823529411765,0.7058823529411765,0.20784313725490197}
\definecolor{color3587b}{rgb}{0.7058823529411765,0.14901960784313725,0.14901960784313725}
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.0939,0.96115)(0.0939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.4439,0.96115)(0.4439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.7939,0.96115)(0.7939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.1439,0.96115)(1.1439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.4939,0.96115)(1.4939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.1939,0.96115)(2.1939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.5439,0.96115)(2.5439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.8939,0.96115)(2.8939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.2439,0.96115)(3.2439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.5939,0.96115)(3.5939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.2939,0.96115)(4.2939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.6439,0.96115)(4.6439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.9939,0.96115)(4.9939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.3439,0.96115)(5.3439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.6939,0.96115)(5.6939,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.0439,0.96115)(6.0439,0.45435)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.1439,0.96115)(8.1439,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.8439,0.96115)(8.8439,0.62935)
\psline[linewidth=0.0212cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(9.1939,0.96115)(9.1939,0.45435)
\psline[linewidth=0.0212cm](0.5369,0.33175)(4.7259,-0.84125)
\psline[linewidth=0.0212cm](1.2355,0.32725)(4.7273,-0.83675)
\psline[linewidth=0.0212cm](2.629,0.31195)(4.7338,-0.82145)
\psline[linewidth=0.0212cm](3.3202,0.29845)(4.7426,-0.80795)
\psline[linewidth=0.0212cm](4.6576,0.26215)(4.8052,-0.77165)
\psline[linewidth=0.0212cm](5.3058,0.26895)(4.857,-0.77845)
\psline[linewidth=0.0212cm](4.9119,-0.84125)(9.1009,0.33175)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.8439,0.96115)(1.8439,0.45435)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.4939,0.96115)(8.4939,0.45435)
\psline[linewidth=0.0219cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.9439,0.96115)(3.9439,0.45435)
\psline[linewidth=0.0219cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.3939,0.96115)(6.3939,0.62935)
\psline[linewidth=0.038cm,linestyle=dotted,dotsep=0.09cm](6.4239,0.52935)(7.9873,0.53275)
\psline[linewidth=0.0219cm](4.0,0.27915)(4.7628,-0.78865)
\psline[linewidth=0.0219cm](1.9332,0.32095)(4.7296,-0.83045)
\psline[linewidth=0.0219cm](4.9105,-0.83675)(8.4023,0.32725)
\psline[linewidth=0.0219cm](5.9756,0.28945)(4.8872,-0.79895)
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.0939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](0.4439,0.3577496){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](0.4439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.7939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](1.1439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](1.1439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](1.4939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](2.1939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](2.5439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](2.5439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](2.8939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](3.2439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](3.2439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](3.5939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](4.2939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](4.6439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](4.6439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](4.9939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](5.3439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](5.3439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](5.6939,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](6.0439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](6.0439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](8.1439,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](8.8439,0.53275){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](9.1939,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](9.1939,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](4.8189,-0.86725){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](8.4939,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](8.4939,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](1.8439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](1.8439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3587b](3.9439,0.35775){0.0939}
\psarc[linewidth=0.010199999,fillstyle=solid,fillcolor=color3588b](3.9439,0.35775){0.0869}{90.0}{270.0}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](6.3939,0.53275){0.0939}
\end{pspicture} 
}
\end{center}



==> figures/gadget.pst.tex <==
% Generated with LaTeXDraw 2.0.2
% Fri Feb 12 09:22:05 CET 2010
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\begin{center}
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.3575)(6.0708,1.3175)
\definecolor{color835b}{rgb}{0.7568627450980392,0.8274509803921568,0.9411764705882353}
\definecolor{color3588b}{rgb}{0.7058823529411765,0.7058823529411765,0.20784313725490197}
\psellipse[linewidth=0.018,dimen=outer,fillstyle=solid,fillcolor=lightgray](0.62285,0.2599999)(0.39399993,0.8539999)
\psline[linewidth=0.018cm](0.6,-0.4025001)(0.38,-0.8025)
\psline[linewidth=0.018cm](0.66,-0.4425)(0.86,-0.8025)
\psline[linewidth=0.018cm](0.62,-0.3825001)(0.62,-0.8425002)
\psframe[linewidth=0.014199999,dimen=outer,fillstyle=solid,fillcolor=lightgray](5.9574,0.8829999)(4.5934,-0.8230002)
\psframe[linewidth=0.014199999,dimen=outer,fillstyle=solid,fillcolor=lightgray](3.5574,0.8829999)(2.1934,-0.8230002)
\psline[linewidth=0.018cm](3.4817,0.9284)(2.9691,1.0565999)
\psline[linewidth=0.018cm](2.2691,0.9284)(2.7817,1.0565999)
\psline[linewidth=0.018cm](2.229,0.8245999)(2.8218,-0.0646002)
\psline[linewidth=0.018cm](2.929,-0.0646002)(3.5218,0.8245999)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.8754,-0.2416)(2.8754,-0.5734)
\psline[linewidth=0.018cm](5.2754,0.9833998)(5.2754,-0.0484001)
\psline[linewidth=0.018cm](4.5913,0.8096999)(4.7345,-0.0497)
\psline[linewidth=0.018cm](5.9595,0.8096999)(5.8163,-0.0497)
\psline[linewidth=0.018cm](4.6691,0.9284)(5.1817,1.0565999)
\psline[linewidth=0.018cm](5.3691,1.0565999)(5.8817,0.9284)
\psline[linewidth=0.018cm](4.9686,0.4663999)(5.2322,0.9936)
\psline[linewidth=0.018cm](5.5822,0.4663999)(5.3186,0.9936)
\psline[linewidth=0.018cm](4.8949,0.2884)(4.7809,-0.0534)
\psline[linewidth=0.018cm](5.6559,0.2884)(5.7699,-0.0534)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.7504,-0.2416)(4.7504,-0.5734)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.2754,-0.2416)(5.2754,-0.5734)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.8004,-0.2416)(5.8004,-0.5734)
\psellipse[linewidth=0.018,dimen=outer,fillstyle=solid,fillcolor=lightgray](2.8754,1.08)(0.1103,0.2375)
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](2.1754,0.9049999){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](3.5754,0.9049999){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](2.8754,-0.1450002){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](4.5754,0.9049999){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](5.9754,0.9049999){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](5.2754,-0.1450002){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](4.7504,-0.1450002){0.0954}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid](5.8004,-0.1450002){0.0954}
\psellipse[linewidth=0.018,dimen=outer,fillstyle=solid,fillcolor=lightgray](5.2754,1.08)(0.1103,0.2375)
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3588b](4.9254,0.3799999){0.0939}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color3588b](5.6254,0.3799999){0.0939}
\psline[linewidth=0.038cm,linestyle=dotted,dotsep=0.09cm](0.62,0.0975)(0.62,-0.4025)
\psline[linewidth=0.018cm](0.1866,0.2353999)(0.5284,0.1213999)
\psline[linewidth=0.018cm](0.153,0.1885998)(0.562,-0.3568)
\psline[linewidth=0.018cm](0.678,-0.3568)(1.087,0.1885998)
\psline[linewidth=0.018cm](1.0534,0.2353999)(0.7116,0.1213999)
\psline[linewidth=0.018cm](0.1866,0.2963999)(0.5284,0.4103999)
\psline[linewidth=0.018cm](0.7116,0.4103999)(1.0534,0.2963999)
\psline[linewidth=0.018cm](0.562,0.8885999)(0.153,0.3431999)
\psline[linewidth=0.018cm](0.678,0.8885999)(1.087,0.3431999)
\psline[linewidth=0.038cm,linestyle=dotted,dotsep=0.09cm](0.62,0.4375)(0.62,0.8892999)
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid,fillcolor=color835b](0.62,-0.4341001){0.095}
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid,fillcolor=color835b](0.62,0.0908998){0.095}
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid](0.095,0.2658999){0.095}
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid](1.145,0.2658999){0.095}
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid,fillcolor=color3588b](0.62,0.4408999){0.095}
\pscircle[linewidth=0.0179,dimen=outer,fillstyle=solid,fillcolor=color3588b](0.62,0.9658998){0.095}
\usefont{T1}{ptm}{m}{n}
\rput(0.54609376,-1.1725){\scriptsize (a)}
\usefont{T1}{ptm}{m}{n}
\rput(2.8160937,-1.1725){\scriptsize (b)}
\usefont{T1}{ptm}{m}{n}
\rput(5.196093,-1.1725){\scriptsize (c)}
\end{pspicture} 
}
\end{center}



==> figures/top.pst.tex <==
% Generated with LaTeXDraw 2.0.2
% Fri Feb 12 09:20:40 CET 2010
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\begin{center}
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.1465)(9.2932,1.1375)
\definecolor{color835b}{rgb}{0.7568627450980392,0.8274509803921568,0.9411764705882353}
\definecolor{color2547b}{rgb}{0.7058823529411765,0.14901960784313725,0.14901960784313725}
\psline[linewidth=0.018cm](4.73,1.0104)(0.1882,-0.5036)
\psline[linewidth=0.018cm](4.7316,1.0057)(0.8866,-0.4989)
\psline[linewidth=0.018cm](4.7343,0.9995)(1.5839,-0.4927)
\psline[linewidth=0.018cm](4.7468,0.9797)(2.9714,-0.4729)
\psline[linewidth=0.018cm](2.2794,-0.4844)(4.7388,0.9912)
\psline[linewidth=0.018cm](4.7623,0.9646)(3.6559,-0.4578)
\psline[linewidth=0.018cm](4.7911,0.9493)(4.3271,-0.4425)
\psline[linewidth=0.018cm](4.8323,0.9449)(4.9859,-0.4381)
\psline[linewidth=0.018cm](4.8685,0.9565)(5.6497,-0.4497)
\psline[linewidth=0.018cm](4.9089,0.9995)(8.0593,-0.4927)
\psline[linewidth=0.018cm](4.9116,1.0057)(8.7566,-0.4989)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.1966,-0.6307)(2.1966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.5466,-0.8057)(2.5466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(2.8966,-0.6307)(2.8966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.2466,-0.8057)(3.2466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.2966,-0.6307)(4.2966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.6466,-0.8057)(4.6466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.9966,-0.6307)(4.9966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.3466,-0.8057)(5.3466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(5.6966,-0.6307)(5.6966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.0466,-0.8057)(6.0466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.1466,-0.6307)(8.1466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.8466,-0.6307)(8.8466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(9.1966,-0.8057)(9.1966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.0966,-0.6307)(0.0966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.4466,-0.8057)(0.4466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.7966,-0.6307)(0.7966,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.1466,-0.8057)(1.1466,-1.1375)
\psline[linewidth=0.018cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.4966,-0.6307)(1.4966,-1.1375)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.8466,-0.8057)(1.8466,-1.1375)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(8.4966,-0.8057)(8.4966,-1.1375)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.5966,-0.6307)(3.5966,-1.1375)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(3.9466,-0.8057)(3.9466,-1.1375)
\psline[linewidth=0.0164cm,linestyle=dashed,dash=0.16cm 0.16cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.3966,-0.6307)(6.3966,-1.1375)
\psline[linewidth=0.038cm,linestyle=dotted,dotsep=0.09cm](6.4266,-0.5425)(8.1666,-0.5425)
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.0966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.7966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](1.4966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](0.4466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](1.1466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](2.8966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](2.1966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](2.5466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](3.2466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](3.5966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](4.2966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](4.6466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](4.9966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](5.6966,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](8.1466,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](5.3466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](6.0466,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](9.1966,-0.7091){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](8.8466,-0.5341){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](1.8466,-0.7091){0.0968}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](8.4966,-0.7091){0.0968}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color2547b](3.9466,-0.7091){0.0939}
\psline[linewidth=0.018cm](4.8066,1.0575)(6.3866,-0.5225)
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](4.8216,1.0409){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](6.3966,-0.5341){0.0945}
%
%
%
\definecolor{color835b}{rgb}{0.7568627450980392,0.8274509803921568,0.9411764705882353}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.3966,0.6084){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.3966,0.2084){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.3966,-0.1916){0.0966}
\pscircle[linewidth=0.0162,dimen=outer,fillstyle=solid,fillcolor=color835b](0.3966,-0.5916){0.0966}
\usefont{T1}{ptm}{m}{n}
\rput(1.7651563,0.59){red - height 5}
\usefont{T1}{ptm}{m}{n}
\rput(2.0426562,0.19){yellow - height 3}
\usefont{T1}{ptm}{m}{n}
\rput(1.8592187,-0.21){blue - height 1}
\usefont{T1}{ptm}{m}{n}
\rput(2.4815626,-0.61){white - height in [1,5]}
\psframe[linewidth=0.04,dimen=outer](4.6,1.0)(0.0,-1.0)
%
%
%
\end{pspicture} 
}
\end{center}


